Object-level Geometric Structure Preserving for Natural Image Stitching

The topic of stitching images with globally natural structures holds paramount significance, with two main goals: pixel-level alignment and distortion prevention. The existing approaches exhibit the ability to align well, yet fall short in maintaining object structures. In this paper, we endeavour to safeguard the overall OBJect-level structures within images based on Global Similarity Prior (OBJ-GSP), on the basis of good alignment performance. Our approach leverages semantic segmentation models like the family of Segment Anything Model to extract the contours of any objects in a scene. Triangular meshes are employed in image transformation to protect the overall shapes of objects within images. The balance between alignment and distortion prevention is achieved by allowing the object meshes to strike a balance between similarity and projective transformation. We also demonstrate that object-level semantic information is necessary in low-altitude aerial image stitching. Additionally, we propose StitchBench, the largest image stitching benchmark with most diverse scenarios. Extensive experimental results demonstrate that OBJ-GSP outperforms existing methods in both pixel alignment and shape preservation. Code and dataset is publicly available at \url{https://github.com/RussRobin/OBJ-GSP}.

==> sec/3_ges-gsppipeline.tex <==
\section{A revisit of stitching pipeline}
\label{sec:ges-gsppipeline}

In this section, we revisit the frequently used stitching pipeline~\cite{gsp}. In the next section we will show how OBJ-GSP preserves object-level structures in this pipeline.
In stitching, a grid mesh is often adopted to guide the image deformation, where $V$ and $E$ represent the sets of vertices and edges within the grid mesh. Image stitching methods aim to find a set of deformed vertex positions, denoted as $\widetilde{V}$, that minimizes the energy function $\psi(V)$.

\textbf{Alignment term} extracts feature points from the input images with the goal of aligning these points after geometric transformation. For each feature point pair $(p, \Phi(p))$, $\widetilde{v}(p)$ represents the position of $p$ as a linear combination of four vertex positions, and $M$ represents the set of all feature point pairs. The algorithm linearly combines the coordinates of the four vertices of each grid to represent the position of $p$ through bi-linear interpolation. By optimizing the positions of grid vertices after geometric transformation, it aims to bring $p$ as close as possible to $\Phi(p)$. Therefore, the energy equation is defined as:

\begin{equation}
\psi_a(V) =  \sum_{p_k \in M} \|   \widetilde{v}(p_k) - \widetilde{v}(\Phi(p_k)) \|^2.
\end{equation}

\textbf{Local similarity term} aims to ensure that the transition from overlapping to non-overlapping regions is natural. Each grid undergoes a similarity transformation to minimize shape distortion. For an edge $(j, k)$, $S_{jk}$ represents its similarity transformation. Suppose $v_j$ transforms to $\widetilde{v_j}$ after deformation, and the energy function is defined as:

\begin{equation}
\psi_l(V) = \sum_{(j,k) \in E_i} \| (\widetilde v_k - \widetilde v_j) - S_{jk}(v_k - v_j) \|^2.
\end{equation}

\textbf{Global similarity term} operates on a global scale to ensure the entire image undergoes a similarity transformation. GSP algorithm evaluates the scale $s$ and rotation $\theta$ within the global image transformation and computes parameters $c(e)$ and $s(e)$ for similarity. Thus, the energy function is defined as:

\begin{equation}
\psi_g(V) = \sum_{e_j \in E} w(e_j)^2[(c(e_j) - s \cos\theta)^2 + (s(e_j) - s \sin\theta)^2].
\end{equation}

\textbf{GES term} in GES-GSP \cite{gesgsp} involves extracting straight lines and curve structures from the image, followed by triangulation to obtain sampled points $\widehat{V_i}$. These points transform to ${\widehat{V_i}}^{desired}$ after projection transformation and similarity transformation. To bring $\widehat{V_i}$ as close as possible to ${\widehat{V_i}}^{desired}$ after the final grid deformation, GES-GSP defines the energy term as:

\begin{equation}
\psi_{ges}(V) = \sum_{\beta = 1}^{N_c} \sum_{\alpha = 1}^{N_s} {\omega_\alpha^\beta E_\alpha^\beta}.
\end{equation}

For a detailed description of the four energy terms mentioned above, please refer to GSP~\cite{gsp} and GES-GSP~\cite{gesgsp} for more information. Ultimately, the sought-after vertices are determined by minimizing the following optimization equation for two images:

\begin{equation}
\widetilde{V} = \text{argmin}_{\widetilde{V}}(\psi_a(\widetilde{V}) + \lambda_l\psi_l(\widetilde{V}) + \psi_g(\widetilde{V}) + \lambda_{ges}\psi_{ges}(\widetilde{V})).
\end{equation}

The above equation represents the optimization for two images. For a scenario involving $n$ images, such as $I_0$, $I_1$, $I_2$, up to $I_{n-1}$, with $I_0$ as the reference image and the remaining $n-1$ images transformed onto the plane of $I_0$, the corresponding energy terms are denoted as $\psi^1$, $\psi^2$, and so on up to $\psi^{n-1}$. The final optimization is performed as:

\begin{equation}
\widetilde{V} = \text{argmin}_{\widetilde{V}}(\psi^1 + \psi^2 + \ldots + \psi^{n-1}).
\end{equation}


==> sec/7_discussion.tex <==
\section{Discussion}
\label{sec:discussion}


\textbf{Limitations:} While OBJ-GSP has demonstrated state-of-the-art performance in image stitching by extracting object-level geometric structures with semantic segmentation and preserving them with triangle mesh sampling, it introduces a large semantic segmentation model into image stitching, resulting in higher computational costs. 
However, with the development of semantic segmentation techniques, lighter versions of SAM will emerge~\cite{efficientsam,lightweightsam}, enhancing the speed of our work.
According to our analysis, the effectiveness of geometric structure extraction significantly impacts the final results. Our method is constrained by the quality of SAM's results. Smaller models like SAM~\cite{sam} with Vit-B/L~\cite{vit} do not perform as SAM with Vit-H. 
Fig.~\ref{fig_ablation} demonstrates the differences.
To stitch a pair of 800*600 images, SAM spends 25s on RTX2090 with 8-24G GPU memory, depending on the backbone. For C++ ONNX implementation, SAM VIT-B spends 1.5 min on CPU.
Mesh optimization and image processing cost less than 4s on an Intel i5 CPU, almost the same as GES-GSP~\cite{gesgsp}.
OBJ-GSP needs more computational resources and time than GES-GSP, but the stitching quality is also better. 
The time cost of SAM is larger than line detection methods in GES-GSP. 
The time used for triangle mesh optimization is almost the same as that in GES-GSP.

\textbf{Applications of OBJ-GSP:}
In many fields, there is a need for high-quality stitched images, even at the expense of long time costs and significant computational resources.
In medical image processing~\cite{medical1,medical2,medical3}, for instance, stitching multiple pathological slice images to reconstruct the entire tissue structure or organ's three-dimensional model demands high precision and quality. These tasks typically necessitate precise alignment and seamless fusion, and can tolerate longer computational times to ensure accuracy. Similarly, in photography~\cite{photography} or virtual tourism~\cite{vt1,vt2} applications, stitching numerous high-resolution images is necessary to generate high-quality panoramic images. This holds true in the fields of remote sensing~\cite{rs1,rs2,rs3} and movie industry~\cite{movie1,movie2} as well.

